Topological strings and Higgsing trees

6-dimensional superconformal field theories are exotic and fascinating. They emerge from compactifications of F-theory on Calabi-Yau elliptic fibrations, which grants them a rich array of dualities with various other formulations of string and M-theory. In this thesis, we consider extended families of elliptic fibrations, giving rise to 6d theories connected by Higgs transitions. These families not only encompass the moduli space of a specific manifold but also include other manifolds with different topologies. Our investigation focuses on rank 1 6D superconformal field theories from two distinct angles. In Chapter 4, we employ modularity, which arises from the holomorphic anomaly equations, to compute the topological string partition function in terms of Jacobi modular forms. We also provide a prescription for obtaining the topological partition function of a Higgsed theory from its parent. Through this approach, we can explain numerous symmetry enhancements that we observed in our study. On the other hand, in Chapter 5, we explore the 2D soliton of the 6D theory, the non-critical string. The elliptic genus of this non-critical string coincides with a part of the topological string partition function. By carefully studying this non-critical string, we propose an ansatz for the elliptic genera expressed in terms of characters of the associated current algebras. We present compelling evidence supporting the validity of this ansatz and unveil novel closed form expressions for the elliptic genera of these non-critical strings. Through these investigations, we hope to shed light on the intriguing world of 6D superconformal field theories and uncover new insights into their remarkable properties and connections.

==> Chapters/Chapter4.tex <==
\chapter{Tools of 2D superconformal theories}

\section{Localization and the JK residue formula}

\section{Elliptic genus}

\section{An example: WZW models}
